QuartDepth: Post-Training Quantization for Real-Time Depth Estimation on the Edge

Monocular Depth Estimation (MDE) has emerged as a pivotal task in computer vision, supporting numerous real-world applications. However, deploying accurate depth estimation models on resource-limited edge devices, especially Application-Specific Integrated Circuits (ASICs), is challenging due to the high computational and memory demands. Recent advancements in foundational depth estimation deliver impressive results but further amplify the difficulty of deployment on ASICs. To address this, we propose QuartDepth which adopts post-training quantization to quantize MDE models with hardware accelerations for ASICs. Our approach involves quantizing both weights and activations to 4-bit precision, reducing the model size and computation cost. To mitigate the performance degradation, we introduce activation polishing and compensation algorithm applied before and after activation quantization, as well as a weight reconstruction method for minimizing errors in weight quantization. Furthermore, we design a flexible and programmable hardware accelerator by supporting kernel fusion and customized instruction programmability, enhancing throughput and efficiency. Experimental results demonstrate that our framework achieves competitive accuracy while enabling fast inference and higher energy efficiency on ASICs, bridging the gap between high-performance depth estimation and practical edge-device applicability. Code: https://github.com/shawnricecake/quart-depth

==> sections/8-rebuttal.tex <==
\newpage 

\newcommand{\red}[1]{\textcolor{red}{\textbf{#1}}}
\newcommand{\green}[1]{\textcolor{green}{\textbf{#1}}}
\newcommand{\blue}[1]{\textcolor{blue}{\textbf{#1}}}
\newcommand{\cyan}[1]{\textcolor{cyan}{\textbf{#1}}}
\newcommand{\magenta}[1]{\textcolor{magenta}{\textbf{#1}}}

%\noindent  Many thanks to the reviewers for the valuable comments. 
\noindent We would like to thank the reviewers for the constructive comments. Below please find our detailed responses.



\noindent \red{$\bullet$ General Response:}
%\jx{\noindent \red{Here, we highlight the contributions and offer some explanations.}}
\textbf{1) Specific designs for depth estimation.} We made in-depth analysis and specific designs for depth estimation. In Sec.~\ref{sec:latency_profiling}, we implement Metric3D on ASIC for latency profiling, which motivates us to focus on quantizing linear and convolution layers in Metric3D. %while   keeping non-linear operations in floating point to preserve accuracy.  
Furthermore, in Sec.~\ref{sec:analysis_distribution}, we visualize  outliers across various channels of an activation in Metric3D, and observe that outliers deviate significantly from the main data  distribution with three peaks (Fig.~\ref{fig:analysis_outlier_distribution}),  different from the discrete outliers at channel level in models for other tasks. To address this, we propose LogNP polishing specifically (Sec.~\ref{sec:activation_polishing}) to polish the distributions with grouped outliers into smooth ones (Fig.~\ref{fig:method_activation_polishing}), different from  general PTQ methods to smooth discrete outliers. 
\textbf{2) Algorithm and Sec.~\ref{sec:compensation}.}
%We will improve the explanations and algorithms in  Sec. 4.2, 4.3 and 4.4.
In Line 201-204,  our framework has three stages in sequential, corresponding to  Sec.~\ref{sec:activation_polishing}, \ref{sec:compensation} and \ref{sec:weight_quant}. %including activation quantization (Sec. 4.2), weight updates to compensate the loss of activation quantization (Section 4.3), and weight quantization for the  updated weights (Section 4.4).  We introduce their detailed computations and steps in the corresponding sections.
In Sec.~\ref{sec:activation_polishing}, activations are quantized following Eq.~\eqref{eq:activation_polishing} with $\alpha$ determined by Eq.~\eqref{eq:activation_polishing_2}.
In the problem formulation of Sec.~\ref{sec:compensation},  the weights are updated with $\Delta W$ so that the layer-wise outputs with quantized  activations $\mathbf{\hat{x}}$ %and updated weights 
should be close to the original output.
We can compute the average $\mathbf{\hat{x}}$ for the whole dataset with the same formulation and optimal solution (Eq.~\eqref{eq:compensation_update}). But it is infeasible   due to the massive dataset size. So we only use a few data samples.  Next in Sec.~\ref{sec:weight_quant}, the updated weights are quantized  by minimizing Eq.~\eqref{eq:F_loss} over trainable quantization parameters with $\textbf{F}_l$ from Eq.~\eqref{eq:KFAC}.
%We will detail the algorithms in the revision.
\jx{We thank the reviewer for their questions and will provide more algorithm details in the revision.}

 
%Then as the activations have been quantized leading to certain quantization errors, we update the weights first to compensate the activation  quantization errors (Sec. 4.3),  and finally perform weight quantization (Sec. 4.4) for the updated weights.  As shown in the problem formulation in Sec. 4.3,  the weights are updated with $\Delta W$ so that the layer-wise outputs with quantized weight activations $\mathbf{\hat{x}}$ and updated weights should be close to the original output. It is infeasible to use the whole dataset or minimize the differences of the model final outputs, due to the massive dataset size or model size. So we only optimize the layer-wise output with a few data samples. We will make this more clear in the revision.  
%For task specific design, we focus on polishing the activations of depth model decoders as shown in the Figure~\ref{fig:analysis_outlier_distribution} (before) and Figure~\ref{fig:method_activation_polishing} (after). The outliers in depth model decoders are grouped and show three peaks in distribution, which is different from those discrete outliers at channel level in models for other tasks.




\noindent \cyan{$\bullet$ Response to Reviewer zr5o}


% 1
% smoothquant, need to revise weight, which makes the weight quantization more difficult
% zeroquant, need more training while we only need calibration
\noindent \textbf{1)} 
% Thanks for including works related to per-channel outliers in activations. 
Smoothquant  needs to revise weights when applying the per-channel smoothing factor according to Eq.(3) in Smoothquant, which makes the weight quantization more difficult as shown in Fig.~\ref{fig:analysis_outlier_distribution} in paper. 
ZeroQuant needs much more training for layer-by-layer knowledge distillation as explained in Appendix B.2 of ZeroQuant while our work only requires calibration without backward.
They focus on discrete outliers in LLMs,  different from our method to address the distributions of  outliers (three different peaks in Fig.~\ref{fig:analysis_outlier_distribution}), which is the main challenge of activation quantization for depth model decoders. Our method successfully  polish three peaks into one (Fig.~\ref{fig:method_activation_polishing}).

% For depth model decoders, the main challenge for activations we solve is polishing three different peaks (Figure~\ref{fig:analysis_outlier_distribution}) into one (Figure~\ref{fig:method_activation_polishing}).

\input{tables/rebuttal_compare_to_fqvit_repvit}
% 2
% we provide the results compared to repqvit
\noindent \textbf{2)} We provide the comparison with FQ-ViT and RepQ-ViT in \textbf{\textcolor{red}{Table~\ref{tab:rebuttal_compare_to_fq_rep}}}. Our method  achieves better performance.
%For RepQ-ViT, we provide the comparison in Table~\ref{tab:rebuttal_compare_to_fq_rep}. 
%Our method achieves better performance than RepQ-ViT.
%\textcolor{red}{(if space available, provide more details about the implementation or experimental setting. it is hard to persuade just with results. More details for how to obtain the results can make it easy to accept.)} 




% 3
% overhead for online polishing (LogNP), @weize
% one table for overhead of online LogNP
\noindent \textbf{3)} 
Clock cycles of GEMM is $(m,k)\times(k,n)$ is $m\times \frac{k}{32}\times \frac{n}{32}$ and Vector is $m\times \frac{n}{32} \times cycles$, where the $32$ is internal parallelism of our GEMM core.
The number of cycles for LogNP in our programmable VCU (detailed in Sec. \ref{sec:on_chip_design}, Line 371-392) cost a total of 12 cycles per vector.
The clock cycles for GEMM and Vector operations with different backbone are shown in \textbf{\textcolor{red}{Table~\ref{tab:rebuttal_cycles}}}.
The Vector computation cycles of LogNP do not exceed the number of cycles required for GEMM.
Benefit from the concurrent execution strategy (Fig.~\ref{fig:instruction}), the overhead  by LogNP can be hidden within GEMM.
\input{tables/rebuttal_cycles}
% In our ASIC design, taking GEMM of $(m,k)\times(k,n)$ as an example, the execution time for GEMM can be calculated as $m\times \frac{k}{k\_group\_size)}\times \frac{n}{n\_group\_size}$, where the $k\_group\_size$ and $n\_group\_size$ is the internal parallelism of our GEMM core.
% As for the time of Vector, it can be calculated by $m\times \frac{n}{n\_group\_size} \times cycles$.
% The number of cycles for the LogNP operation in the VCU cost totaling 12 cycles.
% The time of GEMM and Vector is shown in Table~\ref{tab:rebuttal_cycles}, benefit from the  concurrent execution strategy (shown in Figure~\ref{fig:instruction}), the overhead introduced by LogNP can be fully hidden within GEMM.

% Considering the concurrent execution strategy (shown in Figure~\ref{fig:instruction}), for ViT-small, ViT-large, and ViT-Giant, k is typically set to 384, 1024, and 1536, respectively, and $k\_group\_size$ is set to 32 in our accelerator.
% According to the equation mentioned above, if $\frac{k}{k\_group\_size} \geq cycles$, the time for the Vector operations can be hidden within the GEMM.
% The concurrent strategy shown in Figure~\ref{fig:instruction} overlaps data loading with GEMM and Vector computations. 
% Since data loading time, usually affected by bandwidth, is generally longer than computation time, the LogNP computation in our dataflow will not incur additional overhead.


% 4
% hessian similar to brecq, @pu
\noindent \textbf{4)} Our weight reconstruction  is significantly different from BrecQ.  (i)  
%BRECQ transforms the  second-order error into the change in network outputs characterized by the output Hessian, as shown in its Theorem 3.1. 
Different from BrecQ with transformation to the change of outputs and output (pre-activation) Hessian (its Theorem 3.1), we directly address the second-order error with weight modifications and weight Hessian. (ii) We compute different Hessians with different methods. Our method adopt the KFAC approximation for weight Hessian. Differently, BrecQ approximates the output Hessian with only diagonal elements. (iii) Besides weight quantization, we have other novel contributions, including hardware-related design (Sec.~\ref{sec:analysis_distribution} and~\ref{sec:asic_design}), polishing quantization for activations (Sec.~\ref{sec:analysis_distribution} and~\ref{sec:activation_polishing}) specific for depth estimation, and optimal  compensation for  activation quantization  (Sec.~\ref{sec:compensation}). 



% 5 (minor weakness), paper will benefit if discuss more about LogNP and reconstruction @pu
\noindent \textbf{5) Minor:} Please refer to General Response for  details.





\noindent \magenta{$\bullet$ Response to Reviewer upun}


%Thanks for your review and suggestions for our paper. 

\noindent \textbf{1)} 
We made in-depth analysis and specific designs for depth estimation such as hardware implementation and activation quantization. Please refer to General Response for details. 

\noindent \textbf{2)} Please refer to General Response for details.
 
%Here, we can detail the Section 4.3 and 4.4 here by.. % @pu

% discuss mix precision on ASIC     @weize
% we can support mix precision 4-bit & 8-bit, talk about additional support for mix precision, say it as future research.


\noindent \textbf{3)} % todo: can remove if no space
In the ASIC design flow, all multipliers and adders are custom-designed, which enables support for mix precision.

% arbitrary word lengths in our future research.
\noindent \textbf{4) Minor:} % Thanks for the suggestions of mixed precision strategies and 
We will update the paper according to suggestions. 
% go through the reviewer 2 and talk more about ASIC design







\noindent \blue{$\bullet$ Response to Reviewer zKuM}


% 1
% compare to FQ-ViT and RepQ-ViT
\noindent \textbf{1) More comparison.} %Thanks for the suggestions, 
We provide the comparison with FQ-ViT and RepQ-ViT in Table~\ref{tab:rebuttal_compare_to_fq_rep}. We  perform better. %  than both methods.

% 2
% task specific design is ambigous: mention the LogNP polishing is designed for decoders based on the special distribution shown in Figure~\ref{fig:analysis_outlier_distribution} and 5.
% @ pu, talk more about specific
\noindent \textbf{2) Specific designs.} We made in-depth analysis and specific designs for depth estimation such as hardware and activation quantization.  Please refer to General Response for details. 

%The task specific design in out paper mainly focuses on the LogNP polishing for the depth model decoders. The outliers in decoder activations are grouped as shown in Figure~\ref{fig:analysis_outlier_distribution} rather than discreted. There are three peaks in activation distribution, which makes the activation quantization difficult. With our LogNP polishing, we polish the distributions with grouped outliers into smooth ones, which is different from the methods which smooth discrete outliers in general post-training quantization methods.

\input{tables/rebuttal_ablation_num_cali_samples}
% 3
% ablation study for different number of calibration samples
\noindent \textbf{3) Calibration number.} %Thanks for the discussion of calibration. 
We provide the ablation study for the number of calibration samples in \textcolor{red}{\textbf{Table}}~\ref{tab:rebuttal_ablation_num_calibration_samples}. The results indicate that the model's performance stabilizes when the number of calibration samples reaches 32. Increasing the calibration number  beyond 32 lead to marginal improvements. 
%(e.g., to 64 or 128) does not necessarily improve accuracy and may even result in a slight decline.















==> tables/rebuttal_ablation_num_cali_samples.tex <==

% \begin{table}[]
% \centering
% \resizebox{0.62\linewidth}{!}{
% \begin{tabular}{c|cc|cc}
% \toprule
% Dataset   & \multicolumn{2}{c|}{NYUv2} & \multicolumn{2}{c}{Kitti} \\
% \midrule
% \# Sample & abs\_rel $\downarrow$  & delta1 $\uparrow$  & abs\_rel $\downarrow$  & delta1 $\uparrow$  \\
% \midrule
% \multicolumn{5}{c}{Metric3D with   ViT-Small W4A8}                \\
% \midrule
% 8         & 0.158        & 0.858      & 0.168        & 0.853      \\
% 16        & 0.109        & 0.899      & 0.115        & 0.907      \\
% 32        & 0.103        & 0.899      & 0.092        & 0.916      \\
% 64        & 0.104        & 0.901      & 0.094        & 0.920      \\
% 128       & 0.009        & 0.903      & 0.091        & 0.919      \\
% \midrule
% \multicolumn{5}{c}{Metric3D with   ViT-Small W4A4}                \\
% \midrule
% 8         & 0.201        & 0.792      & 0.259        & 0.465      \\
% 16        & 0.140        & 0.801      & 0.217        & 0.493      \\
% 32        & 0.133        & 0.815      & 0.197        & 0.534      \\
% 64        & 0.137        & 0.821      & 0.189        & 0.528      \\
% 128       & 0.132        & 0.818      & 0.192        & 0.531     \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-3.5mm}
% \caption{Ablation study for number of calibration samples.}
% \label{tab:rebuttal_ablation_num_calibration_samples}
% \vspace{-8mm}
% \end{table}



\begin{table}[htp]
\centering
\scriptsize
\vspace{-4mm}
\setlength{\tabcolsep}{3pt}
\scalebox{0.8}{
\begin{tabular}{c|cc|cc|cc|cc}
\toprule
Dataset   & \multicolumn{2}{c|}{NYUv2} & \multicolumn{2}{c|}{Kitti} & \multicolumn{2}{c|}{NYUv2} & \multicolumn{2}{c}{Kitti} \\
\# Sample & abs\_rel $\downarrow$  & delta1 $\uparrow$  & abs\_rel $\downarrow$  & delta1 $\uparrow$  & abs\_rel $\downarrow$  & delta1 $\uparrow$  & abs\_rel $\downarrow$  & delta1 $\uparrow$  \\
\midrule
W / A     & \multicolumn{4}{c|}{Metric3D with ViT-Small W4A8}      & \multicolumn{4}{c}{Metric3D with ViT-Small W4A4}      \\
\midrule
8         & 0.158        & 0.858      & 0.168        & 0.853      & 0.201        & 0.792      & 0.259        & 0.465      \\
16        & 0.109        & 0.899      & 0.115        & 0.907      & 0.140        & 0.801      & 0.217        & 0.493      \\
32        & 0.103        & 0.899      & 0.092        & 0.916      & 0.133        & 0.815      & 0.197        & 0.534      \\
64        & 0.104        & 0.901      & 0.094        & 0.920      & 0.137        & 0.821      & 0.189        & 0.528      \\
128       & 0.009        & 0.903      & 0.091        & 0.919      & 0.132        & 0.818      & 0.192        & 0.531     \\
\bottomrule
\end{tabular}
}
\vspace{-3.5mm}
\caption{Ablation study for number of calibration samples.}
\label{tab:rebuttal_ablation_num_calibration_samples}
\vspace{-4mm}
\end{table}








==> tables/rebuttal_compare_to_fqvit_repvit.tex <==
\begin{comment}
\begin{table}[]
\vspace{-9mm}
\centering
\scriptsize
\setlength{\tabcolsep}{1pt}
\scalebox{0.8}{
\begin{tabular}{c|c|cc|cc}
\toprule
\multicolumn{2}{c}{Dataset} & \multicolumn{2}{c|}{NYUv2} & \multicolumn{2}{c}{Kitti} \\
\midrule
Method         & W / A      & abs\_rel $\downarrow$  & delta1 $\uparrow$  & abs\_rel $\downarrow$  & delta1 $\uparrow$  \\
\midrule
\multicolumn{6}{c}{Metric3D with   ViT-Small Backbone}                              \\
\midrule
FQ-ViT         & W4A8       & 0.227        & 0.617      & 0.269        & 0.446      \\
RepQ-ViT       & W4A8       & 0.418        & 0.219      & 0.404        & 0.228      \\
Ours           & W4A8       & \textbf{0.103}        & \textbf{0.899}      & \textbf{0.092}        & \textbf{0.916}      \\
\midrule
FQ-ViT         & W4A4       & 0.365        & 0.366      & 0.637        & 0.021      \\
RepQ-ViT       & W4A4       & 0.439        & 0.316      & 0.517        & 0.125      \\
Ours           & W4A4       & \textbf{0.133} & \textbf{0.815} & \textbf{0.197} & \textbf{0.534} \\
\midrule
\multicolumn{6}{c}{Metric3D with   ViT-Large Backbone}                              \\
\midrule
FQ-ViT         & W4A8       & 0.535        & 0.319      & 0.304        & 0.425      \\
RepQ-ViT       & W4A8       & 0.327        & 0.537      & 0.691        & 0.184      \\
Ours           & W4A8       & \textbf{0.071} & \textbf{0.970} & \textbf{0.055} & \textbf{0.973} \\
\midrule
FQ-ViT         & W4A4       & 0.958        & 0.183      & 0.501        & 0.134      \\
RepQ-ViT       & W4A4       & 0.541        & 0.302      & 0.837        & 0.002      \\
Ours           & W4A4       & \textbf{0.097} & \textbf{0.932} & \textbf{0.070} & \textbf{0.952} \\
% \midrule
% \multicolumn{6}{c}{Depth Anything with   ViT-Large Backbone}                        \\
% \midrule
% FQ-ViT         & W4A8       & 0.478        & 0.341      & 0.287        & 0.418      \\
% RepQ-ViT       & W4A8       & 0.389        & 0.519      & 0.625        & 0.192      \\
% Ours           & W4A8       & \textbf{0.058} & \textbf{0.982} & \textbf{0.060} & \textbf{0.965} \\
% \midrule
% FQ-ViT         & W4A4       & 0.921        & 0.174      & 0.455        & 0.209      \\
% RepQ-ViT       & W4A4       & 0.439        & 0.278      & 0.761        & 0.018      \\
% Ours           & W4A4       & \textbf{0.070} & \textbf{0.972} & \textbf{0.059} & \textbf{0.935} \\
\bottomrule
\end{tabular}
}
\vspace{-3.5mm}
\caption{Compare to FQ-ViT and RepQ-ViT.}
\vspace{-8mm}
\label{tab:rebuttal_compare_to_fq_rep}
\end{table}
\end{comment}

\begin{table}[t]
% \vspace{-4mm}
\centering
\scriptsize
\setlength{\tabcolsep}{1pt}
\scalebox{0.8}{
\begin{tabular}{c|c|cc|cc|c|cc|cc}
\toprule
Dataset & & \multicolumn{2}{c|}{NYUv2} & \multicolumn{2}{c|}{Kitti} & & \multicolumn{2}{c|}{NYUv2} & \multicolumn{2}{c}{Kitti}\\
& W / A      & abs\_rel $\downarrow$  & delta1 $\uparrow$  & abs\_rel $\downarrow$  & delta1 $\uparrow$   & W / A  & abs\_rel $\downarrow$  & delta1 $\uparrow$  & abs\_rel $\downarrow$  & delta1 $\uparrow$ \\
\midrule
Method & \multicolumn{5}{c|}{Metric3D with ViT-Small Backbone} & \multicolumn{5}{c}{Metric3D with ViT-Large Backbone}  \\
\midrule
FQ-ViT         & W4A8       & 0.227        & 0.617      & 0.269        & 0.446      & W4A8       & 0.535        & 0.319      & 0.304        & 0.425      \\
RepQ-ViT       & W4A8       & 0.418        & 0.219      & 0.404        & 0.228      & W4A8       & 0.327        & 0.537      & 0.691        & 0.184      \\
Ours           & W4A8       & \textbf{0.103}        & \textbf{0.899}      & \textbf{0.092}        & \textbf{0.916}      & W4A8       & \textbf{0.071} & \textbf{0.970} & \textbf{0.055} & \textbf{0.973} \\
\midrule
FQ-ViT         & W4A4       & 0.365        & 0.366      & 0.637        & 0.021      & W4A4 & 0.958        & 0.183      & 0.501        & 0.134      \\
RepQ-ViT       & W4A4       & 0.439        & 0.316      & 0.517        & 0.125      & W4A4 & 0.541        & 0.302      & 0.837        & 0.002      \\
Ours           & W4A4       & \textbf{0.133} & \textbf{0.815} & \textbf{0.197} & \textbf{0.534} & W4A4 & \textbf{0.097} & \textbf{0.932} & \textbf{0.070} & \textbf{0.952} \\
% \midrule
% \multicolumn{6}{c}{Depth Anything with   ViT-Large Backbone}                        \\
% \midrule
% FQ-ViT         & W4A8       & 0.478        & 0.341      & 0.287        & 0.418      \\
% RepQ-ViT       & W4A8       & 0.389        & 0.519      & 0.625        & 0.192      \\
% Ours           & W4A8       & \textbf{0.058} & \textbf{0.982} & \textbf{0.060} & \textbf{0.965} \\
% \midrule
% FQ-ViT         & W4A4       & 0.921        & 0.174      & 0.455        & 0.209      \\
% RepQ-ViT       & W4A4       & 0.439        & 0.278      & 0.761        & 0.018      \\
% Ours           & W4A4       & \textbf{0.070} & \textbf{0.972} & \textbf{0.059} & \textbf{0.935} \\
\bottomrule
\end{tabular}
}
\vspace{-3.5mm}
\caption{Compare to FQ-ViT and RepQ-ViT.}
\vspace{-7mm}
\label{tab:rebuttal_compare_to_fq_rep}
\end{table}


==> tables/rebuttal_cycles.tex <==
% \begin{table}[]
% \vspace{-9mm}
% \centering
% \resizebox{0.6\linewidth}{!}{%
% \begin{tabular}{cccc}
% \toprule
% \multicolumn{1}{c|}{Res.} & \multicolumn{1}{c|}{Dim}                   & \multicolumn{1}{c|}{GEMM Cycles} & Vector Cycles \\ \midrule
% \multicolumn{4}{c}{ViT-Small}                                                                                             \\ \midrule
% \multicolumn{1}{c|}{256}  & \multicolumn{1}{c|}{\multirow{3}{*}{384}}  & \multicolumn{1}{c|}{36,864}       & 36,864         \\
% \multicolumn{1}{c|}{512}  & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{73,728}       & 73,728         \\
% \multicolumn{1}{c|}{1024} & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{147,456}      & 147,456        \\ \midrule
% \multicolumn{4}{c}{ViT-Large}                                                                                             \\ \midrule
% \multicolumn{1}{c|}{256}  & \multicolumn{1}{c|}{\multirow{3}{*}{1024}} & \multicolumn{1}{c|}{262,144}      & 98,304         \\
% \multicolumn{1}{c|}{512}  & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{524,288}      & 196,608        \\
% \multicolumn{1}{c|}{1024} & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{1,048,576}     & 393,216        \\ 
% \midrule
% \multicolumn{4}{c}{ViT Giant}                                                                                             \\ \midrule
% \multicolumn{1}{c|}{256}  & \multicolumn{1}{c|}{\multirow{3}{*}{1536}} & \multicolumn{1}{c|}{589,824}      & 147,456        \\
% \multicolumn{1}{c|}{512}  & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{1,179,648}     & 294,912        \\
% \multicolumn{1}{c|}{1024} & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{2,359,296}     & 589,824        \\ 
% \bottomrule
% \end{tabular}%
% }
% \vspace{-3.5mm}
% \caption{The Number of cycles for GEMM and Vector.}
% \label{tab:rebuttal_cycles}
% \vspace{-3.5mm}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htp]
\centering
\vspace{-4mm}
\scriptsize
\setlength{\tabcolsep}{3pt}
\scalebox{0.9}{
\begin{tabular}{c|c|c|c}
\toprule
Model         & ViT-Small & ViT-large & ViT-Giant \\ \midrule
Dimension     & 384       & 1024      & 1536      \\ 
Resolution    & 1024      & 1024      & 1024      \\ \midrule
GEMM Cycles   & 147,456   & 1,048,576 & 2,359,296 \\
Vector Cycles & 147,456   & 393,216   & 589,824   \\ 
\bottomrule
\end{tabular}%
}
\vspace{-3.5mm}
\caption{The Number of cycles for GEMM and Vector.}
\label{tab:rebuttal_cycles}
\vspace{-4mm}
\end{table}
